Descriptive set theory and forcing; How to prove theorems about Borel sets the hard way

These are lecture notes from a course I gave at the University of Wisconsin during the Spring semester of 1993. Part 1 is concerned with Borel hierarchies. Section 13 contains an unpublished theorem of Fremlin concerning Borel hierarchies and MA. Section 14 and 15 contain new results concerning the lengths of Borel hierarchies in the Cohen and random real model. Part 2 contains standard results on the theory of Analytic sets. Section 25 contains Harrington's Theorem that it is consistent to have $\Pi^1_2$ sets of arbitrary cardinality. Part 3 has the usual separation theorems. Part 4 gives some applications of Gandy forcing. We reverse the usual trend and use forcing arguments instead of Baire category. In particular, Louveau's Theorem on $\Pi^0_\alpha$ hyp-sets has a simpler proof using forcing.

==> README.tex <==
%auto-ignore
% Logic Eprints
%Submitted 1554 Wed Jan 12, 1994 by: miller@math.wisc.edu (arnold miller )
%logic/miller/dstforce
%logic/miller/dstforce/shar1
%logic/miller/dstforce/shar2

The main file is called "main.tex" curiously enough.
It calls all the other files.
It is written in standard LaTeX (version 2.09) except
for the definitions in "kludge.tex".  This defines
Bbb (blackboard bold face), goth (gothic), and special
characters from the AMS.  If you don't have these
fonts edit the first few lines of kludge.tex.
The standard macros are in macdef.tex.

It probably should be run 3 times thru latex before
the table of contents settles down to the correct page
numbers.

%%%%%%%% index.tex
Because different TeX's break lines differently, the
index entries may be off a page or two. The file index.tex
was produced by using the file main.idx which is created by
latex.  I put the staggering in by hand (after machine sort)
and then machine sorted that on column 20.
main.idx >>
  replace ? by \
  sort
  indent 13
  stagger
  sort on column 25
>> index.tex

%%%%%%%%% bib.tex
The file cite.tex is produced by the macro \site which writes
to cite.tex the page number where the the paper is cited.
Page numbers are joined to bibin.tex to produce bib.tex.

After settling on page numbers
cite.tex,bibin.tex >>
run bib2.bat
>> bib.tex





==> bibin.tex <==
%auto-ignore

\begin{thebibliography}{99}

\bibitem{addison}
J.W.Addison, Separation principles in the hierarchies of classical
and effective descriptive set theory, Fundamenta Mathematicae, 46(1959),
123-135.

\bibitem{addison2}
J.W.Addison, Some consequences of the axiom of constructibility,
Fundamenta Mathematicae, 46(1957), 337-357.

\bibitem{baire}
R.Baire, Sur la repr\'{e}sentation des fonctions discontinues (2me partie),
Acta Mathematica, 32(1909), 97-176.

\bibitem{balogh}
Z.Balogh, There is a $Q$-set space in ZFC,
Proceedings of the American Mathematical Society,  113(1991), 557-561.

\bibitem{barto4}
T.Bartoszynski, Combinatorial aspects of measure and category,
Fundamenta Mathematicae, 127(1987), 225-239.

\bibitem{barto}
T.Bartoszynski, On covering of real line by null sets,
Pacific Journal of Mathematics, 131(1988),1-12.

\bibitem{barto2}
T.Bartoszynski, S.Shelah,
The cofinality of cardinal invariants related to measure and category,
Journal of Symbolic Logic, 54(1989),  719-726.

\bibitem{barto3}
T.Bartoszynski, H.Judah,
On the cofinality of the smallest covering of the real line by meager sets,
Journal-of-Symbolic-Logic, 54(1989), 828-832.

\bibitem{barwise}
J.Barwise, {\bf Admissible sets and structures}, Springer-Verlag, 1975.

\bibitem{bell}
M.Bell, On the combinatorial principal P(c), Fundamenta Mathematicae,
114(1981), 149-157.

\bibitem{bbm}
R.H.Bing, W.W.Bledsoe, R.D.Mauldin, Sets generated by rectangles,
Pacific J. Math., 51(1974, 27-36.

\bibitem{brez}
C.Brezinski, {\bf History of Continued Fractions and Pad\'{e} Approximants},
Springer-Verlag, 1991.

\bibitem{burgess}
J.Burgess, Infinitary languages and descriptive set theory, PhD
University of California, Berkeley, 1974.

\bibitem{burgess2}
J.Burgess, Equivalences generated by families of Borel sets, Proceedings
of the American Mathematical Society, 69(1978), 323-326.

\bibitem{burgess3}
J.Burgess, Effective enumeration of classes in a $\Sigma^1_1$ equivalence
relation, Indiana University Mathematics Journal, 28(1979), 353-364.

\bibitem{ems}
F.van Engelen,  A.Miller, J.Steel, Rigid Borel sets and
better quasiorder theory, Contemporary Mathematics
(American Mathematical Society), 65(1987), 199-222.

\bibitem{euler}
L.Euler, De fractionibus continuis dissertatio, Comm.Acad.Sc.Imp.St.
P\'{e}tersbourg, 9(1737), 98-137.

\bibitem{ekm}
F.van Engelen, K.Kunen, A.Miller, Two remarks about analytic sets,
Lecture Notes in Mathematics, Springer-Verlag, 1401(1989), 68-72.

\bibitem{erdkm}
P.Erdos, K.Kunen, R.Mauldin,
Some additive properties of sets of real numbers,
Fundamenta Mathematicae, 113(1981), 187-199.

\bibitem{feng}
Q.Feng, Homogeneity for open partitions of pairs of reals, to appear
in TAMS.


\bibitem{qsets}
W.Fleissner, A.Miller,  On Q-sets, Proceedings of the American
Mathematical Society, 78(1980), 280-284.

\bibitem{fleiss1}
W.Fleissner,
Current research on $Q$ sets,
in {\bf Topology, Vol. I (Proc. Fourth Colloq., Budapest, 1978)},
Colloq. Math. Soc. Janos Bolyai, 23(1980), 413-431.

\bibitem{fleiss2}
W.Fleissner, Squares of $Q$ sets,
Fundamenta Mathematicae, 118(1983), 223-231.

\bibitem{fremlin}
D.H.Fremlin, On the Baire order problem, Note of 29.4.82.

\bibitem{frembook}
D.H.Fremlin, {\bf Consequences of Martin's Axiom}, Cambridge University
Press, 1984.

\bibitem{fried}
H.Friedman, PCA well-orderings of the line, Journal of Symbolic Logic,
39(1974), 79-80.


\bibitem{frieds}
S.Friedman, Steel Forcing and Barwise compactness,
Annals of Mathematical Logic, 22(1982), 31-46.

\bibitem{galmil}
F.Galvin, A.Miller, $\gamma$-sets and other singular sets of real
numbers, Topology and Its Applications, 17(1984), 145-155.

\bibitem{gandy}
R.O.Gandy, Proof of Mostowski's conjecture,
Bulletin de L'Academie Polonaise des Science, 8 (1960), 571-575.

\bibitem{god}
K.G\"odel, The consistency of the axiom of choice and of the
generalized continuum hypothesis, Proceedings of the National
Academy of Science, 24(1938), 556-557.

\bibitem{harrsilv}
L.Harrington, A powerless proof of a Theorem of Silver,
handwritten note dated 11-76.

\bibitem{harlouv}
L.Harrington, Theorem (A. Louveau), handwritten note undated,
circa 1976.

\bibitem{harring}
L.Harrington, Long projective well-orderings,
Annals of Mathematical Logic, 12(1977), 1-24.

\bibitem{harrsharp}
L.Harrington, Analytic determinacy and $0^{\#}$,
Journal of Symbolic Logic, 43(1978), 685-693.

\bibitem{harsami}
L.Harrington, R.Sami,
Equivalence relations, projective and beyond, Logic Colloquium 78,
ed Boffa et al, North Holland 1979, 247-263.

\bibitem{harrshel}
L.Harrington and S.Shelah, Counting equivalence classes for
co-$\kappa$-Sous\-lin equivalence relations, in {\bf Logic Colloquium 80},
North-Holland, 1982.


\bibitem{harshemar}
L.Harrington, D.Marker, S.Shelah, Borel orderings,
Transactions-of-the-American-Mathematical-Society,  310(1988), 293-302.

\bibitem{hinman}
P.Hinman, {\bf Recursion-Theoretic Hierarchies}, Springer-Verlag, 1978.

\bibitem{jech}
T.Jech, {\bf Set Theory}, Academic Press, 1978.

\bibitem{jensol}
R.B.Jensen, R.M.Solovay, Some applications of almost disjoint sets,
in {\bf Mathematical Logic and Foundations of Set Theory},
ed by
Y.Bar-Hillel, 1970, North-Holland, 84-104.

\bibitem{qsetzero}
 H.Judah, S.Shelah,
 $Q$-sets do not necessarily have strong measure zero,
 Proceedings of the American Mathematical Society,  102 (1988), 681-683.

\bibitem{qsetsier}
H.Judah, S.Shelah, $Q$-sets, Sierpinski sets, and rapid filters,
Proceedings of the American Mathematical Society,  111(1991), 821-832.

\bibitem{kondo}
M.Kond\v{o}, Sur l'uniformisation des compl\'{e}mentaires analytiques et
les ensembles projectifs de la seconde classe, Japan J. Math. 15(1939),
197-230.

\bibitem{kecref}
A. Kechris,
Spector second order classes and reflection,
in {\bf Generalized recursion theory, II }, North-Holland 1978,
Studies Logic Foundations Math.,  94(1978), 147-183.


\bibitem{kechris2}
A.Kechris, On transfinite sequences of projective sets with an application
to ${\bf\Sigma}^1_2$ equivalence
relations, in {\bf Logic Colloquium '77} ed by Macintyre et al,
North-Holland, 1978, 155-160.

\bibitem{kechris3}
A. Kechris,
The perfect set theorem and definable wellorderings of the continuum,
Journal of Symbolic Logic, 43(1978),
630-634.

\bibitem{kecmar}
A.S.Kechris, D.A.Martin, Infinite games and effective descriptive
set theory, in {\bf Analytic sets}, ed by C.A.Rogers, Academic
Press, 1980.

\bibitem{kechris}
A.S.Kechris, {\bf Lectures on classical descriptive set theory},
to appear.

\bibitem{kleene}
S.Kleene, Hierarchies of number-theoretic predicates, Bulletin of
the American Mathematical Society, 63(1955), 193-213.

\bibitem{kunmil}
K. Kunen, A.Miller, Borel and projective sets from the point of view of
compact sets, Mathematical Proceedings of the Cambridge Philosophical
Society, 94(1983), 399-409.

\bibitem{kunenma}
K.Kunen,
Where MA first fails,
Journal-of-Symbolic-Logic, 53(1988),  429-433.

\bibitem{kur}
K.Kuratowski, {\bf Topology}, vol 1, Academic Press, 1966.


\bibitem{kurmos}
K.Kuratowski, A.Mostowski, {\bf Set theory, with an introduction to
descriptive set theory}, North-Holland, 1976.

\bibitem{landver}
A.Landver,
Singular $\sigma$-dense trees,
Journal-of-Symbolic-Logic, 57(1992), 1403-1416.

\bibitem{landver2}
A.Landver,
Baire numbers, uncountable Cohen sets and perfect-set forcing,
Journal-of-Symbolic-Logic, 57(1992), 1086-1107.

\bibitem{leb}
H.Lebesgue, Sur les fonctions repr\'{e}sentables  analytiquement,
Journal de Math\'{e}matiques Pures et Appliqu\'{e}s, 1(1905), 139-216.

\bibitem{louvsilv}
A. Louveau,
Relations d'equivalence dans les espaces polonais,
Collection: General logic seminar, (Paris, 1982--83), 113-122,
Publ. Math. Univ. Paris VII.


\bibitem{louveau}
A.Louveau, A separation theorem for $\Sigma^1_1$ sets,
Transactions of the American Mathematical Society, 260(1980), 363-378.

\bibitem{loust}
A.Louveau, J.Saint Raymond, Borel classes and closed games: Wadge-type
and Hurewicz-type results, Transactions of the American Mathematical
Society, 304(1987), 431-467.

\bibitem{louvlin}
A. Louveau, Two results on Borel orders,
Journal of Symbolic Logic, 54(1989),  865-874.

\bibitem{louvbor}
A.Louveau, Classifying Borel Structures, in
{\bf Set Theory of the Continuum}, ed by Judah et al.,
Springer-Verlag, 1992, 103-112.

\bibitem{luz}
N.Luzin, Sur un probl\`eme de M. Baire, Comptes Rendus Hebdomaddaires Seances
Academie Science Paris, 158(1914), 1258-1261.

\bibitem{mahlo}
P.Mahlo, \"Uber Teilmengen des Kontinuums von dessen Machtigkeit,
Sitzungsberichte der Sachsischen Akademie der Wissenschaften zu Leipsiz,
Mathematisch-Naturwissenschaftliche Klasse 65, (1913), 283-315.

\bibitem{manfield}
R.Mansfield,  The non-existence of $\Sigma^1_2$ well-ordering of
the Baire space, Fundamenta Mathematicae, 86(1975), 279-282.

\bibitem{mansf}
R.Mansfield, Perfect subsets of definable sets of real numbers,
Pacific Journal of Mathematics, 35(1970), 451-457.

\bibitem{manweit}
R.Mansfield, G.Weitkamp, {\bf Recursive Aspects of Descriptive Set
Theory},  Oxford University Press (1985).


\bibitem{marsol}
D.A.Martin, R.M.Solovay,  Internal Cohen extensions,
Annals of Mathematical Logic, 2(1970), 143-178.

\bibitem{borelhier}
A.Miller, On the length of Borel hierarchies, Annals of Mathematical Logic,
16(1979), 233-267.



\bibitem{cat}
A.Miller, On generating the category algebra and the Baire order problem,
Bulletin de L'Academie Polonaise des Science, 27(1979), 751-755.

\bibitem{gensous}
A.Miller, Generic Souslin sets, Pacific Journal of Mathematics,
97(1981), 171-181.
\bibitem{someprop}
A.Miller, Some properties of measure and category, Transactions of
the American
Mathematical Society, 266(1981), 93-114. Corrections and additions to
some properties of measure and category, Transactions of the American
Mathematical Society, 271(1982), 347-348.

\bibitem{ctlbcof}
A.Miller, The Baire category theorem and cardinals of countable cofinality,
Journal of Symbolic Logic, 47(1982), 275-288.

\bibitem{char}
A.Miller, A characterization of the least cardinal for which the Baire category
theorem fails, Proceedings of the American Mathematical Society, 86(1982),
498-502.

\bibitem{maponto}
A.Miller,  Mapping a set of reals onto the reals, Journal of Symbolic Logic,
48(1983), 575-584.

\bibitem{ctblmod}
A.Miller, The Borel classification of the isomorphism class of a
countable model,
Notre Dame Journal of Formal Logic, 24(1983), 22-34.

\bibitem{survey1}
A.Miller, Special subsets of the real line,
in {\bf Handbook of set-theoretic topology},
North Holland, 1984, 201-233.

\bibitem{prikmil}
A.Miller, K. Prikry, When the continuum has cofinality $\omega_1$,
Pacific Journal of Mathematics, 115(1984), 399-407.

\bibitem{infcomb}
A.Miller, Infinite combinatorics and definability,
Annals of Pure and Applied Mathematical Logic, 41(1989), 179-203.

\bibitem{proj}
A.Miller, Projective subsets of separable metric spaces,
Annals of Pure and Applied Logic, 50(1990), 53-69.


\bibitem{survey2}
A.Miller, Special sets of reals, in {\bf Set Theory of the Reals},
ed Haim Judah, Israel Mathematical Conference Proceedings,
vol 6(1993), 415-432, American Math Society.

\bibitem{playful}
Y.Moschovakis, Uniformization in a playful universe, Bulletin of
the American Mathematical Society, 77(1971), 731-736.

\bibitem{mosch}
Y.Moschovakis, {\bf Descriptive set theory}, North-Holland 1980.

\bibitem{pop}
G.Poprougenko, Sur un probl/`{e}me de M. Mazurkiewicz, Fundamenta
Mathematicae, 15(1930), 284-286.

\bibitem{przym}
T.Przymusinski, The existence of $Q$-sets is
equivalent to the existence of strong $Q$-sets,
Proceedings of the American Mathematical Society, 79(1980), 626-628.

\bibitem{anal}
C.A.Rogers
et al, editors, {\bf Analytic Sets}, Academic Press, 1980.

\bibitem{roth}
F.Rothberger, On some problems of Hausdorff and of Sierpinski,
Fundamenta Mathematicae, 35(1948), 29-46.

\bibitem{sack}
G.Sacks, {\bf Higher Recursion Theory}, Springer-Verlag, 1990.

\bibitem{sami}
R.Sami, On $\Sigma_1^1$ equivalence relations with Borel
classes of bounded  rank,
Journal of Symbolic Logic, 49(1984),  1273-1283.

\bibitem{shelah}
S. Shelah, On co-$\kappa $-Souslin relations,
Israel Journal of Mathematics, 47(1984),  139-153. |

\bibitem{shoen}
J.Shoenfield, The problem of predicativity, Essays on the foundations
of mathematics, Magnes press, Hebrew University, Jerusalem, 1961,
132-139.

\bibitem{sierp1928}
W.Sierpinski, {\bf Introduction to general topology},
University of Toronto Press, 1934, translated from original
Polish version of 1928.


\bibitem{sikor}
R. Sikorski, {\bf Boolean Algebras}, Springer-Verlag New York,
1969, 3rd edition.

\bibitem{silver}
J.Silver, Counting the number of equivalence classes of Borel
and coanalytic  equivalence relations,
Annals-of-Mathematical-Logic, 18(1980), 1-28.

\bibitem{Solecki}
S.Solecki, Covering analytic sets by families of closed sets, preprint
1993.

\bibitem{solov}
R.M.Solovay, On the cardinality of $\Sigma^1_2$ sets of reals, in
{\bf Foundations of Mathematics}, Biulof et al eds., Springer-Verlag
(1969), 58-73.

\bibitem{solten}
R.M.Solovay, S.Tennenbaum, Iterated Cohen extensions and Souslin's problem,
Annals of Mathematics, 94(1971), 201-245.

\bibitem{spector}
C.Spector, Hyperarithmetical quantifiers, Fundamenta Mathematicae,
48(1960), 313-320.

\bibitem{marcz}
E.Spilrajn, Sur l'\'{e}quivence des suites d'ensembles et
l'\'{e}quivence des fonctions, Fundamenta Mathematicae, 26(1936),
302-326.

\bibitem{marcz2}
E.Spilrajn, The characteristic function of a sequence of sets
and some of its applications, Fundamenta Mathematicae, 31(1938),
207-223.

\bibitem{steel}
J.R.Steel, Forcing with tagged trees,
Annals of Mathematical Logic, 15(1978), 55-74.

\bibitem{stern}
J.Stern,
Perfect set theorems for analytic and coanalytic equivalence relations,
in {\bf Logic Colloquium '77} ed by Macintyre et al,
North-Holland, 1978, 277-284.

\bibitem{stern2}
J. Stern,
Effective partitions of the real line into Borel sets of bounded rank,
Annals of Mathematical Logic, 18 (1980), 29-60.


\bibitem{will}
S.Williard, {\bf General Topology}, Addison-Wesley, 1970.


\end{thebibliography}












==> cite.tex <==
baire 6
sierp1928 8
sierp1928 8
euler 8
brez 8
will 11
leb 11
leb 13
ctblmod 13
addison 13
bbm 14
proj 16
survey2 16
marcz 17
marcz2 17
marcz2 17
borelhier 17
roth 20
jensol 20
marsol 20
bell 21
galmil 21
qsets 21
frembook 21
fleiss1 21
fleiss2 21
survey1 21
survey2 21
przym 21
qsetzero 21
qsetsier 21
balogh 21
borelhier 23
steel 30
frieds 30
harrsharp 30
silver 30
jech 31
borelhier 32
sikor 36
borelhier 37
borelhier 37
sikor 38
mahlo 39
luz 39
mahlo 39
borelhier 39
borelhier 40
marsol 41
solten 43
prikmil 44
cat 45
borelhier 51
borelhier 52
fremlin 53
galmil 54
kunmil 58
qsetzero 59
maponto 60
pop 67
maponto 74
someprop 74
borelhier 74
ctlbcof 75
barto 77
barto2 77
barto3 77
ctlbcof 77
ctlbcof 78
kunenma 79
frembook 79
landver 79
landver2 79
barto4 79
char 79
anal 80
kur 80
mosch 80
god 84
addison2 84
shoen 88
shoen 89
mansf 90
solov 90
kondo 92
playful 96
kurmos 96
solov 97
marsol 97
manfield 99
kechris3 99
fried 99
harring 100
harring 103
kleene 106
hinman 108
barwise 108
spector 111
gandy 111
erdkm 114
infcomb 114
ems 114
silver 115
harrsilv 115
kecmar 115
manweit 115
louvsilv 115
harrshel 115
harshemar 120
ekm 122
ekm 122
Solecki 124
harshemar 124
harshemar 124
louvlin 124
louvbor 124
feng 125
burgess 126
burgess2 130
burgess3 130
harsami 130
sami 130
stern 130
stern2 130
kechris2 130
harrshel 130
shelah 130
harshemar 130
louveau 131
loust 132
kechris 134
harshemar 138
kecref 138
harlouv 142
sack 142
manweit 142


==> grading.tex <==
%auto-ignore
\begin{center}
  Grading
\end{center}

At MIT apparently they also have to have a minimum number of
graduate students in a course for it to run. Here we need at least
eight. They say that Norbert Wiener at MIT would start every graduate
course no matter what the title or topic with two weeks of adding,multiplying
complex numbers- done slowly and simply.  After two weeks a course
will run no matter what-so again no matter what the title or topic
of the course Wiener would immediately launch into an exposition of
his latest research paper- usually losing most of the class.

\bigskip

Well enough of this, lets get started.

$$   (2 + 3i)(5 + 7i)=?  $$

\bigskip

Grading policy:  In order to get an A

\begin{center}
  Not required
\end{center}
\begin{enumerate}
\item exams- there will be none
\item homework- there will be none
\item attendance- encouraged but not required
\item reading the notes
\item membership in the human species
\item living being
\end{enumerate}

\begin{center}
  Required
\end{center}
\begin{enumerate}
\item you must be registered
\item you must be able to multiply complex numbers\footnote{Apparently
I was too strict, the class started
with about ten and ended with only three students regularly attending.}
\item you must laugh at the instructors jokes\footnote{
On a course evaluation:
`I've taken this course five times and this one was the worst!'
What can I say? It hurts to be slammed by an expert.-Aaron Meyerowitz}
\end{enumerate}



